Evolution of the Water Snow Line in Magnetically Accreting Protoplanetary Disks

The low water content of the terrestrial planets in the solar system suggests that the protoplanets formed within the water snow line. Accurate prediction of the snow line location moving with time provides a clue to constrain the formation process of the planets. In this paper, we investigate the migration of the snow line in protoplanetary disks whose accretion is controlled by laminar magnetic fields, which have been proposed by various nonideal magnetohydrodynamic (MHD) simulations. We propose an empirical model of the disk temperature based on our nonideal MHD simulations, which show that the accretion heating is significantly less efficient than in turbulent disks, and calculate the snow line location over time. We find that the snow line in the magnetically accreting laminar disks moves inside the current Earth's orbit within 1 Myr after star formation, whereas the time for the conventional turbulent disk is much longer than 1 Myr. This result suggests that either the rocky protoplanets formed in such an early phase of the disk evolution, or the protoplanets moved outward to the current orbits after they formed close to the protosun.

==> diff_preamble.tex <==
% inserted from diff_preamble.tex

%DIF FONTSTRIKE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf} %DIF PREAMBLE
\providecommand{\DIFaddtex}[1]{{\bf #1}} %DIF PREAMBLE
\providecommand{\DIFdeltex}[1]{{\footnotesize \sout{#1}}} %DIF PREAMBLE
%DIF COLOR PREAMBLE %DIF PREAMBLE
\RequirePackage{color} %DIF PREAMBLE
\providecommand{\DIFaddbegin}{\protect\color{blue}} %DIF PREAMBLE
\providecommand{\DIFaddend}{\protect\color{black}} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{\protect\color{red}} %DIF PREAMBLE
\providecommand{\DIFdelend}{\protect\color{black}} %DIF PREAMBLE
\providecommand{\DIFmodbegin}{} %DIF PREAMBLE
\providecommand{\DIFmodend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF HYPERREF PREAMBLE %DIF PREAMBLE
\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}} %DIF PREAMBLE

